Rec4Ad: A Free Lunch to Mitigate Sample Selection Bias for Ads CTR Prediction in Taobao

Click-Through Rate (CTR) prediction serves as a fundamental component in online advertising. A common practice is to train a CTR model on advertisement (ad) impressions with user feedback. Since ad impressions are purposely selected by the model itself, their distribution differs from the inference distribution and thus exhibits sample selection bias (SSB) that affects model performance. Existing studies on SSB mainly employ sample re-weighting techniques which suffer from high variance and poor model calibration. Another line of work relies on costly uniform data that is inadequate to train industrial models. Thus mitigating SSB in industrial models with a uniform-data-free framework is worth exploring. Fortunately, many platforms display mixed results of organic items (i.e., recommendations) and sponsored items (i.e., ads) to users, where impressions of ads and recommendations are selected by different systems but share the same user decision rationales. Based on the above characteristics, we propose to leverage recommendations samples as a free lunch to mitigate SSB for ads CTR model (Rec4Ad). After elaborating data augmentation, Rec4Ad learns disentangled representations with alignment and decorrelation modules for enhancement. When deployed in Taobao display advertising system, Rec4Ad achieves substantial gains in key business metrics, with a lift of up to +6.6\% CTR and +2.9\% RPM.

==> src/related.tex <==
\section{Related Work}
In this section, we summarize studies related to CTR prediction and selection bias in ranking systems.

Existing CTR models mainly focus on capturing feature interactions between users and items for prediction. Wide\&Deep~\cite{cheng2016wide}, DeepFM~\cite{guo2017deepfm} and xDeepFM~\cite{lian2018xdeepfm} combine both low-order and high-order interactions to enhance model expressiveness. PNN~\cite{qu2016product} captures inter-field interactions with a product layer. Bing~\cite{ling2017model} uses a Neural Network boosted with GBDT ensemble model. To specifically handle behavior sequences containing rich information about user interest, DIN~\cite{zhou2018deep} adopts the attention mechanism to aggregate historical behaviors. SIM~\cite{pi2020search} explicitly filter lifelong sequences with category information of target items. Though above methods have achieved encouraging performance, they fail to consider selection bias in ads ctr prediction and thus can be further improved.

In recent years, many research efforts are proposed to handle various kinds of biases in ranking systems, such as position bias~\cite{wang2018position}, conformity bias~\cite{zheng2021disentangling}, trust bias~\cite{agarwal2019addressing}, and selection bias~\cite{wang2016learning,ovaisi2020correcting,pmlr-v48-schnabel16,uniform20,yuan2019improving,si2022model}. Studies on selection bias can be divided into two groups. The first group is based on Inverse Propensity Scoring (IPS), which re-weights samples according to their impression propensity.  For example, Wang et al.~\cite{wang2016learning} propose 
query-dependent bias models for selection bias in search engines. Ovaisi et al.~\cite{ovaisi2020correcting} adapts Heckman’s correction method to estimate the probability of a document being observed. Schnabel et al.~\cite{pmlr-v48-schnabel16} proposes to estimate propensities with techniques like Naive Bayes and Logistic Regression. Though theoretically unbiased, IPS-based methods usually suffer from the problem of high-variance~\cite{bottou2013counterfactual,zheng2021disentangling}. More importantly, sample-reweighting potentially change label distribution of displayed items, which could yield un-calibrated predictions that are prohibited in ads CTR models. The second group relies on uniform data collected with random policy. For example, Yuan et al.~\cite{yuan2019improving} train an unbiased imputation model based on uniform data,  which helps predict labels on non-displayed items for data augmentation. Liu et al.~\cite{uniform20} propose to eliminate selection bias by knowledge distillation from unbiased models. However, collection of uniform data is usually at the cost of user experience and platform revenue. Moreover, the obtained uniform data of this
magnitude is far from enough to train industrial models with billions of parameters. By contrast, our proposed Rec4Ad leverages recommendations samples which widely co-exist with ad samples and mitigates selection bias via disentangled representation learning, making it a practical and effective framework for ads ctr prediction in industrial systems.



